Constraining SN Ia Progenitors from the Observed Fe-peak Elemental Abundances in the Milky Way Dwarf Galaxy Satellites

Chemical abundances of iron-peak elements in the red giants of ultra-faint dwarf galaxies (UFD) and dwarf spheroidal galaxies (dSph) are among the best diagnostics in the cosmos to probe the origin of Type Ia Supernovae (SNe Ia). We incorporate metallicity-dependent SN Ia nucleosynthesis models for different progenitor masses in our inhomogeneous galactic chemical evolution model, {\tt{i-GEtool}}, to recreate the observed elemental abundance patterns and their spread in a sample of UFD and dSph galaxies with different average metallicities and star formation histories. Observations across different environments indicate that [Mn/Mg] increases on average with metallicity while [Ni/Mg] remains nearly constant. The average dispersion of [X/Mg] from our UFD model ranges between $0.20$ and $0.25$ for iron-peak elements, with the exception of [Sc/Mg] that has $\sigma \approx 0.39$. Chemical evolution models assuming Chandrasekhar mass (M$_{\text{Ch}}$) SN Ia progenitors produce similar [Mn/Mg]-[Fe/H] and [Ni/Mg]-[Fe/H] abundance patterns to those observed in the examined UFD and dSph galaxies, without the need to invoke a substantial fraction of sub-M$_{\text{ch}}$ progenitors that change across different environments, as claimed by some previous chemical evolution studies. Sub-M$_{\text{ch}}$ progenitors in our dSph models under produce both [Ni/Mg]-[Fe/H] and [Ni/Mg]-[Fe/H] abundance patterns, with the $1\,\text{M}_{\odot}$ sub-M$_{\text{ch}}$ model explaining a number of outliers in [Ni/Mg]-[Fe/H], while the outliers in [Mn/Mg]-[Fe/H] require higher sub-M$_{\text{ch}}$ progenitor masses.

==> readme.tex <==
% readme.txt
%
% MNRAS journal LaTeX package
% v3.2 for LaTeX 2e
%
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `author-maintained'.
% 
% The Current Maintainer of this work is: Royal Astronomical Society,
% MNRAS Editorial Office, who can be contacted on mn@ras.ac.uk
%
% This work consists of all the files listed in readme.txt
%
%
% Last updated 20 July 2023
%
% Copyright (C) Royal Astronomical Society 2021, Blackwell Science 2001,
% Cambridge University Press 1994
%
% See each file for a detailed author list and change log.
%
% This package consists of the following files:

readme.txt          This file

mnras.cls           MNRAS LaTeX document class
mnras.bst           MNRAS BibTeX style

mnras_guide.tex     User guide, LaTeX format
mnras_guide.pdf     User guide, PDF format
mnras_template.tex  A simple template paper

example.eps         An example image used in the guide
example.png         An example image used in the guide
example.ps          An example image used in the guide

legacy\legacy.txt   Description of the legacy releases
legacy\mn2e.cls     v2.2 of mn2e.cls (deprecated)
legacy\mn2e.bst     v1.1b of mn2e.bst (deprecated)


% Disclaimer:
%
% This LaTeX package is provided free to the community in the hope that it
% assists them in preparing papers for the journal Monthly Notices of the
% Royal Astronomical Society.
% The files are provided 'as-is' with no guarantee of their suitability,
% freedom from errors or omissions, or compatibility with any software.
% The Royal Astronomical Society cannot provide user support for this package,
% LaTeX, or for any other software.
% Authors are free to use other styles or programmes if they wish.
% Please see the journal instructions to authors for guidance.
% This disclaimer is in addition to the No Warranty section of the licence,
% at the link given above.
